Mixture-Models: a one-stop Python Library for Model-based Clustering using various Mixture Models

\texttt{Mixture-Models} is an open-source Python library for fitting Gaussian Mixture Models (GMM) and their variants, such as Parsimonious GMMs, Mixture of Factor Analyzers, MClust models, Mixture of Student's t distributions, etc. It streamlines the implementation and analysis of these models using various first/second order optimization routines such as Gradient Descent and Newton-CG through automatic differentiation (AD) tools. This helps in extending these models to high-dimensional data, which is first of its kind among Python libraries. The library provides user-friendly model evaluation tools, such as BIC, AIC, and log-likelihood estimation. The source-code is licensed under MIT license and can be accessed at \url{https://github.com/kasakh/Mixture-Models}. The package is highly extensible, allowing users to incorporate new distributions and optimization techniques with ease. We conduct a large scale simulation to compare the performance of various gradient based approaches against Expectation Maximization on a wide range of settings and identify the corresponding best suited approach.

==> Autodiff.tex <==
\section{Automatic Differentiation}
\label{app:AD}
The contents of this section are from our previous work \cite{KASA202267}, with examples from
\cite{baydin2018automatic}.


	One way to fit a statistical model on data is to infer parameters that maximize the probability of observing the data - this procedure is called Maximum Likelihood Estimation (MLE). Local optima of the likelihood function can be found through standard gradient ascent procedure.
	In traditional gradient-based inference, gradients are required in closed form which becomes laborious or intractable to derive as the model complexity increases. 
	To automate the computation of derivatives three classes of techniques have been developed:
	\begin{enumerate}[(i)]
		\item 
		Symbolic Differentiation (SD): evaluates derivatives in closed-form by means of symbolic manipulations and reduction using rules of differential calculus. 
		\item
		Numerical differentiation (ND): numerical values of the gradients are evaluated using approximations based on finite differences, interpolation and other numerical methods.
		\item
		Automatic Differentiation or Algorithmic Differentiation (AD): numerical values of the exact gradients are evaluated to machine precision by the use of computational graphs and elementary arithmetic operations, without requiring closed form expressions.
	\end{enumerate}
	
	
	AD has become the workhorse for optimization routines in machine learning today due to its numerical accuracy and the ease of implementation it affords.
	The original ideas of AD date back to \cite{nolan1953analytical,beda1959programs} with major improvements decades later by \cite{griewank1989automatic}. 
	A historical overview can be found in \cite{rall2006perspectives}.
	Some previous statistical models have used AD for optimization. 
	Examples include non-linear random effects models by \cite{fournier2012ad,skaug2006automatic,skaug2002automatic} and Bayesian models \citep{kucukelbir2017automatic}.
	We outline the key ideas of AD in the following;
	more details can be found in  \cite{,verma2000introduction,baydin2018automatic,margossian2019review}.
	
	
	The numerical computation of a function can be decomposed into a finite set of operations. This decomposition, also called evaluation trace of the function or Wengert list \citep{wengert1964simple}, can be formed by means of intermediary variables and elementary operations.
	These operations most commonly include arithmetic operations and transcendental function evaluations.
	AD numerically computes the derivative of a function by combining the derivatives of the elementary operations and propagating Taylor series coefficients through the systematic application of the chain rule of differential calculus.
	The efficiency of the computation is improved by storing evaluated values of intermediate sub-expressions that may be re-used.
	
	
	
	As an example, consider the following differentiable function, $f(x_1,x_2) = x_1^2 \sin(x_2)$.  
	This function %
	can be decomposed into its evaluation trace 
	as follows:
	
	$$\begin{array}{c}
	t_{1}=x_{1} \\
	t_{2}=x_{2} \\
	t_{3}=t_{1} \times t_{1} \\
	t_{4}=\sin \left(t_{2}\right) \\
	t_{5}=t_{3} \times t_{4}
	\end{array}
	$$
	
	In the above decomposition, the intermediary variables corresponding to the Wengert list of the function $f$ are $t_3$ and $t_4$. The computation of $f$  can be represented by a \textit{computational graph} where square nodes represent variables and circular nodes represent the intermediate elementary operations:
	
	\begin{figure}[!h]
		\centering
		\tikzset{every picture/.style={line width=0.75pt}} %
		
		\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1,scale=0.8]
		
		\draw   (200,95) .. controls (200,85.06) and (208.06,77) .. (218,77) .. controls (227.94,77) and (236,85.06) .. (236,95) .. controls (236,104.94) and (227.94,113) .. (218,113) .. controls (208.06,113) and (200,104.94) .. (200,95) -- cycle ;
		\draw   (145,153) .. controls (145,142.51) and (153.51,134) .. (164,134) .. controls (174.49,134) and (183,142.51) .. (183,153) .. controls (183,163.49) and (174.49,172) .. (164,172) .. controls (153.51,172) and (145,163.49) .. (145,153) -- cycle ;
		\draw   (251,151.5) .. controls (251,141.28) and (259.28,133) .. (269.5,133) .. controls (279.72,133) and (288,141.28) .. (288,151.5) .. controls (288,161.72) and (279.72,170) .. (269.5,170) .. controls (259.28,170) and (251,161.72) .. (251,151.5) -- cycle ;
		\draw   (146,212) -- (183,212) -- (183,249) -- (146,249) -- cycle ;
		\draw    (163.8,213.4) -- (163.99,174) ;
		\draw [shift={(164,172)}, rotate = 450.28] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
		
		\draw    (175.4,138.2) -- (200.93,106.95) ;
		\draw [shift={(202.2,105.4)}, rotate = 489.25] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
		\draw    (258.2,137.4) -- (232.74,109.28) ;
		\draw [shift={(231.4,107.8)}, rotate = 407.84000000000003] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
		\draw    (218,77) -- (217.82,59.4) ;
		\draw [shift={(217.8,57.4)}, rotate = 449.42] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
		\draw   (251.5,210.5) -- (288.5,210.5) -- (288.5,247.5) -- (251.5,247.5) -- cycle ;
		\draw    (269.3,211.9) -- (269.49,172.5) ;
		\draw [shift={(269.5,170.5)}, rotate = 450.28] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
		
		
		\draw (164.21,150.46) node  [rotate=-0.32]  {${\wedge}^{2}$};
		\draw (257.8,143.2) node [anchor=north west][inner sep=0.75pt]    {$sin$};
		\draw (209,86.4) node [anchor=north west][inner sep=0.75pt]    {$\times $};
		\draw (213.6,35.2) node [anchor=north west][inner sep=0.75pt]    {$f$};
		\draw (156.4,225.1) node [anchor=north west][inner sep=0.75pt]    {$x_{1}$};
		\draw (261.9,225.1) node [anchor=north west][inner sep=0.75pt]    {$x_{2}$};
		
		
		\end{tikzpicture}
		
		\caption{Computational Graph}
		\label{fig:computational_graph}
	\end{figure}
	
	Now each step of this composition can be individually evaluated for gradients, with respect to each independent variable, using simple rules of differentiation as follows:
	
	$$
	\begin{array}{l}
	\nabla t_{1}=(1,0) \\
	\nabla t_{2}=(0,1) \\
	\nabla t_{3}=2 \times t_{1} \times \nabla t_{1} \\
	\nabla t_{4}=\cos \left(t_{2}\right) \times \nabla t_{2} \\
	\nabla t_{5}=t_{3} \times \nabla t_{4}+t_{4} \times \nabla t_{3}
	\end{array}
	$$
	
	Thus, for a given value of $(x_1,x_2)$, we can compute the exact value of the gradient of the function $\nabla f = \nabla t_{5}$. 
	The process of constructing the computational graphs and propagating the gradients at each step is automated by AD tools using source-code transformation  or operator overloading. Source-code transformation generates an augmented
	code in which all specified partial derivatives are computed in addition to the original result for an input function.
	In operator overloading, the semantics of elementary operators are changed in the compiler to accommodate partial derivative computations as well.
	Derivative computation may be done in forward or reverse mode, and can be specified in the AD tool.
	In forward mode, the independent variable is fixed and the derivative of each sub-expression is computed recursively. 
	In reverse mode, which is more efficient, the dependent variable is fixed and the derivative with respect to each sub-expression is computed recursively. 
	They are essentially the chain rule applied in different order.
	Backpropagation, used to train neural networks, is a special case of reverse mode AD.
	
	Efficient implementations of AD are available in several programming languages and frameworks, e.g. Python \citep{maclaurin2015autograd}, R \citep{pav2016madness}, PyTorch \citep{paszke2017automaticfull} and Stan \citep{carpenter2015stan}.
	Many first and second order gradient-based optimization algorithms are implemented in these libraries that use AD as black-box solvers.
	
	\subsection{Expression Swell in SD}
	
	
	To compute gradients by hand, we first evaluate the complete expression and then differentiate it using rules of differential calculus. 
	First note that a naive computation may repeatedly evaluate the same expression multiple times, e.g., consider the rules:
	\begin{align}
	\frac{d}{dx} \left(A(x) + B(x)\right) \leadsto \frac{d}{dx} A(x) + \frac{d}{dx} B(x) \\
	\frac{d}{dx} \left(A(x)\,B(x)\right) \leadsto \left(\frac{d}{dx} A(x)\right) B(x) + A(x) \left(\frac{d}{dx} B(x)\right)
	\label{ecostat_appendix:EquationMultiplicationRule}
	\end{align}
	
	Let $H(x)=A(x)B(x)$. 
	Note that $H(x)$ and $\frac{d}{dx}H(x)$ have in  common: $A(x)$ and $B(x)$, 
	and on the right hand side, $A(x)$ and $\frac{d}{dx}A(x)$ appear separately. 
	In symbolic differentiation we plug the derivative of $A(x)$ and thus 
	have nested duplications of any computation that appears in common between $A(x)$ and $\frac{d}{dx}B(x)$. 
	In this manner symbolic differentiation can produce exponentially large symbolic expressions which take correspondingly long to evaluate. This problem is called expression swell.
	To illustrate the problem, consider the following 
	example from  \cite{baydin2018automatic}.
	The logistic map is defined recursively as $l_{n+1}=4l_n (1-l_n)$, $l_1=x$. We want to computed the derivatives of $l_n$ with respect to $x$ for different values of $n$.
	Table \ref{ecostat_appendix:TableExpressionSwell} clearly shows that the number of repetitive evaluations increase with $n$.
	
	\begin{table}[!h]
		\centering
		\captionof{table}{Iterations of the logistic map $l_{n+1}=4l_n (1-l_n)$, $l_1=x$ and the corresponding derivatives of $l_n$ with respect to $x$, illustrating expression swell 
			(from \cite{baydin2018automatic}) }
		\label{ecostat_appendix:TableExpressionSwell}
		\renewcommand{\arraystretch}{1}
		
		{\small
			\begin{tabularx}{\columnwidth}{@{}lXp{3cm}XX@{}}
				\toprule
				$n$ & $l_n$ & $\frac{d}{dx}l_n$ & $\frac{d}{dx}l_n$ (Simplified form)\\
				\addlinespace
				\midrule
				1 & $x$ & $1$ & $1$\\
				2 & $4x(1 - x)$ & $4(1 - x) -4x$ & $4 - 8x$\\
				3 & $16x(1 - x)(1 - 2 x)^2$ & $16(1 - x)(1 - 2 x)^2 - 16x(1 - 2 x)^2 - 64x(1 - x)(1 - 2 x)$ & $16 (1 - 10 x + 24 x^2 - 16 x^3)$\\
				4 & $64x(1 - x)(1 - 2 x)^2$ $(1 - 8 x + 8 x^2)^2$ & $128x(1 - x)(-8 + 16 x)(1 - 2 x)^2 (1 - 8 x + 8 x^2) + 64 (1 - x)(1 - 2 x)^2  (1 - 8 x + 8 x^2)^2 - 64x(1 - 2 x)^2 (1 - 8 x + 8 x^2)^2 - 256x(1 - x)(1 - 2 x)(1 - 8 x + 8 x^2)^2$ & $64 (1 - 42 x + 504 x^2 - 2640 x^3 + 7040 x^4 - 9984 x^5 + 7168 x^6 - 2048 x^7)$\\
				\bottomrule
		\end{tabularx}}
	\end{table}
	
	If the symbolic form is not required and only numerical evaluation of derivatives is required, computations can be simplified by storing the values of intermediate sub-expressions.
	Further efficiency gains in computation can be achieved by interleaving differentiation and simplification steps.
	The derivative of $l_{n+1} = 4 l_{n} (1- l_{n})$ can be found using the chain rule $\frac{dl_{n+1}}{dl_n}\frac{dl_{n}}{dl_{n-1}}\dots \frac{dl_{1}}{dl_x}$ which simplifies to $4(1-l_{n} - l_{n})4(1-l_{n-1} - l_{n-1})\dots4(1-x - x)$. 
	Note that evaluation in AD is computationally linear in $n$ (because we add only one $(1-l_n - l_n)$ for each increase by 1).
	This linear time complexity is achieved due to `carry-over' of the derivatives at each step, rather than evaluating the derivative at the end and substituting the value of x. 
	
	The Python code below shows the simplicity of the implementation for this problem.
	
	
	
	
	\begin{center}
		\begin{verbatim}
		from autograd import grad
		def my_func(x,n):
		p = x
		y = x * (1 - x)
		for i in range(n):
		y = y*(1 - y)
		
		return y
		grad_func = grad(my_func)
		grad_func(0.5,4)
		\end{verbatim}
	\end{center}
	
	
	\subsubsection*{Comparison of ND, SD and AD}
	
	Through the use of the computational graphs and exact computation of derivatives, AD overcomes the limitations of both SD and ND.
	AD is faster and more accurate compared to ND that uses numerical approximations. 
	ND is easy to implement but is slow at high dimensions and often results in floating point errors.
	
	The run time, computational complexity and memory requirements of SD do not scale with increasing number of parameters. 
	Moreover, it cannot be used for functions that are defined using programmatic constructs such as conditions and loops.
	Note that
	SD first obtains the closed-form expression through symbolic manipulations and then evaluates it whereas AD bypasses the derivation of the closed form and directly evaluates the derivative of the function.
	This yields substantial advantages with respect to the running time.
	
	To illustrate this advantage in runtime, consider the following recursive expressions: 
	$l_0 = \frac{1}{1+e^x}$, $l_1 = \frac{1}{1+e^{l_0}} $, ....., $l_{n} = \frac{1}{1+e^{l_{n-1}}}.$
	We evaluate the derivative of $l_{n}$ with respect to $x$ and compare the runtime in Mathematica (SD) vs PyTorch (AD) for various values of $n$. As $n$ increases, it is expected that runtime also increases. It can be seen from the results in Table \ref{Runtime}  that runtime increases linearly for AD (using PyTorch) whereas it increases exponentially for SD (using Mathematica).  
	\begin{table}[t]
		\begin{center}
			\begin{tabular}{ ccc } 
				\toprule
				n & \text{AD}  & \text{SD} \\ \midrule
				1 & 0.00013 & 0.00000 \\ 
				5 & 0.00030 & 0.00005 \\ 
				10 & 0.00051 & 0.00023 \\
				50 & 0.00293 & 0.00437 \\
				100 & 0.00433 & 0.15625 \\
				200 & 0.00917 & 1.45364 \\
				\bottomrule
			\end{tabular}
		\end{center}
		\captionof{table}{Average runtime (over 1000 runs) }
		\label{Runtime}
	\end{table}

